Revealing the True Indicators: Understanding and Improving IoC Extraction From Threat Reports

Indicators of Compromise (IoCs) are critical for threat detection and response, marking malicious activity across networks and systems. Yet, the effectiveness of automated IoC extraction systems is fundamentally limited by one key issue: the lack of high-quality ground truth. Current extraction tools rely either on manually extracted ground truth, which is labor-intensive and costly, or on automated ground truth creation methods that include non-malicious artifacts, leading to inflated false positive (FP) rates and unreliable threat intelligence. In this work, we analyze the shortcomings of existing ground truth creation strategies and address them by introducing the first hybrid human-in-the-loop pipeline for IoC extraction, which combines a large language model-based classifier (LANCE) with expert analyst validation. Our system improves precision through explainable, context-aware labeling and reduces analysts' work factor by 43% compared to manual annotation, as demonstrated in our evaluation with six analysts. Using this approach, we produce PRISM, a high-quality, publicly available benchmark of 1,791 labeled IoCs from 50 real-world threat reports. PRISM supports both fair evaluation and training of IoC extraction methods and enables reproducible research grounded in expert-validated indicators.

==> Chapters/SuplemetnaryMaterial.tex <==


\section{LANCE Prompts}
\label{app:LANCEPrompts}

This section presents the prompt engineering phase for LANCE as well as the evaluation of the final prompts. For both the prompt engineering phase and the evaluation of the prompts, we used ChatGPT 4o \cite{GPT4o} as the underlying LLM. 

\subsection{Prompt engineering and Input structuring}

To evaluate prompt performance, we manually extracted and labeled all indicators in 10 reports. These reports were selected from AlienVault with the turgent of ensuring diversity in structure, size, and IoC density. The indicator extraction and labeling process was iterative, as some indicators were missed or misclassified in the initial extraction iteration.

We conducted 27 structured prompt tests to refine our approach. Initially, we tested prompts that processed the entire report while simultaneously targeting all IoC types. However, this resulted in poor performance, including high confusion and inconsistency in model responses. This behavior has been well documented in the bibliography \cite{InstructionFinetuning,ZeroShot,DecomposePrompting}.To address this, we modified the prompt structure to classify each IoC type separately, leading to more reliable and consistent results. 

Each iteration involved reviewing model outputs for false positives and false negatives. Based on observed errors, we adjusted prompts for each IoC type to address recurring misclassifications. 

Due to the nature of the different types of indicators, as well as the reasons for appearing in a report, some types were more difficult to prompt than others. Specifically, domain labeling was the most difficult task to prompt-engineer for. In our experiments, we came across several domain-like strings that were not actual domains. This was to be expected if taking into consideration the results in Figure \ref{fig:fp_fn_combined}. In addition, the appearance of nonIoC domains in IoC URLs was very common, making it necessary for the prompt to cover these instances of domains. 

The second most difficult type was URLs. The difficulty of labeling URLs arose from the fact that in several cases, there were placeholders in the extracted URLs, as they were included in the threat report as examples. Even though the obvious cases could easily be tackled with rule-based implementations, there were several cases where the example/placeholder part of the URL was not obvious or representable by a specific rule. Thus, we needed to find a way to describe the problem to the model and request it to label as ``nonIoC'' these URLs.

The prompts for IPs, and file hashes were easily engineered in early iterations of the process.

During our tests, there were some occasions when we found that the prompt engineering was not enough to tackle the problem at hand, so we implemented other techniques, such as the rolling window input. We chose the size of 8000 characters as this is close to the maximum number of tokens the model can output. Even though a token can include more than one character, we wanted to make sure that in cases where all 8000 characters were a list of important strings (e.g., Hashes), the model would be able to output them properly with their label. To make sure that no information would be lost due to the splitting of the report, we implemented an overlap of 50\% in each consecutive report segment. 

The techniques analyzed in Section~\ref{subsec:LLMmethodology} as well as the corresponding parts from the final prompt used for URLs, can be seen in Table~\ref{tab:Prompt}. By constructing our prompts this way, we address most of the pitfalls the LLM can fall into and steer it away from common inaccuracies.




\begin{table*}[h]
    \centering
    \begin{tabular}{lll}
        \hline
        \textbf{Prompt Technique} & \textbf{Description} & \textbf{Example} \\
        \hline
        Role specification  & Specification of the role that the LLM is & You are a cybersecurity analyst.  
        \\
        & expected to take.  & 
        
        \\
        
        Input definition  & Clear definition of what the input is.  & I will give you part of a cybersecurity report along
        \\ & & with some URLs found in that section.  
        
        \\
        
        Task definition & Clear definition of the classification task.  & Your Task is to label each of the given URLs as ether ``IoC'' 
        \\ & & or ``nonIoC'' based on the context that the URL is given \\ & & in the report. 
        
        \\
        
        Definition of Terms  & Explicit definitions of what constitutes an & Label as ``IoC'' the URLs that are Indicators
        \\ &  ``IoC'' vs. a ``nonIoC''.  &  of Compromise (IoCs) related to malicious activities,
        \\ & & such as phishing, malware, or other cyber threats, and as 
        \\ & & ``nonIoC'' if they are not referenced in the context of IoCs.  
        
        \\
        
        Reference to common & Examples, and references to common False &If a given URL is not complete (eg. is split by a new line or 
        \\
        mistakes &  Positives and False Negatives. & has a placeholder), do not label it as an IoC. 
        \\ & & Do not return URLs that were not in the given list, but make 
        \\ & & sure that you return all the URLs in the given list. I want you 
        \\ & & to make sure that the number of URLs in the ``Extracted URLs''
        \\ & & list that I give you is the same as the number of URLs \\ & & you return. 
        
        \\
        
        Secondary task definition & Clear definition of the justification task. & I also want you to justify your choice of the label for each URL. 
        
        \\
        
        Thoroughness Reminder & Reminder to process the report carefully and thoroughly, & Go through the report part twice to make sure
        \\ & encouraging multiple passes over the text. &  your labeling and justifications are correct. 
        \\ & & Make sure that for each URL you followed all the given \\ & & instructions.
        
        \\
        
        Output format request & Specification for the expected output format to ensure & Return all the URLs, their label, and the justification
        \\ &  parseability and downstream usability. &  separated by ``,'' , one per line, with no additional text. 
        \\ & &  The list might be empty, in that case, return an empty output.
        \\

        
        


        \hline
    \end{tabular}
    \caption{Performance metrics (P5, P10, P20, P40, P50) for different indicator types based on pairs of Analysts in part 1. Each column represents the maximum average agreement on reports that are in that percentile. }
    \label{tab:Prompt}
\end{table*}

\subsection{Prompt evaluation}
\label{subsec:PromptEval}

For the evaluation of the automated IoC extraction pipeline, we collected the 10 most recent reports added to the AlienVault database from their original user profile. We then manually extracted and labeled the indicators that existed in the text of the reports to create our test dataset.

We evaluated the Precision, Recall, and F1 score of LANCE and compared them with IoC Searcher. The evaluation can be seen in Figure \ref{fig:promt_eval}. The Recall of both LANCE and IoC Searcher was 100\% in all types of IoCs and in total.


\begin{figure}[ht]
    \centering
    
    \includegraphics[width=\linewidth]{plots/precision_f1_stacked.pdf}
    
    \caption{This figure compares the precision and F1 score of LANCE and the rule-based IoC Searcher across multiple IoC types. The LANCE consistently achieves higher precision and F1, particularly on domains and URLs. The values above each bar indicate the exact performance for each indicator type and overall.}
    
    \label{fig:promt_eval}
\end{figure}


\section{User Interface}
\label{app:UI}

Figures \ref{fig:UI1} and \ref{fig:UI2} show a view of the custom user interface developed for our system. In the proposed user interface (Figure~\ref{fig:UI2}), the analyst can see all indicators highlighted by a red or green rectangle. In the cases that the LANCE-generated label is \textit{IoC}, the rectangle is red, while if the label is \textit{nonIoC} it is green. This way, the analyst can quickly understand the generated label. By hovering over the indicator or by selecting the indicator, they can see the justification that LANCE provided for the selected label.  The label of each indicator can be changed by the analyst either by selecting the indicator and clicking the designated button or by double-clicking the indicator. The label change propagates to all instances of this indicator throughout the report. 

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{UI22.png}
    \caption{This is a view of the User Interface the Analysts
    used for part 2 of the Ground Truth creation. Contrary to
    the User Interface for Part 1, the indicators are extracted and
    labeled by the LLM pipeline. The Indicators labeled as IoC
    can be seen in a red rectangle, while those labeled as nonIoC
    can be seen in a green rectangle. A justification is provided
    for all indicators.
    }
    \label{fig:UI2}
\end{figure*}

For the baseline annotation pass (BAP), the user interface was altered to not show the designated colors unless the label was assigned by the analyst. The analyst could also not see the label, justification, or any other LANCE-generated information about any indicator. For this pass, we also implemented a counter that showed the remaining unlabeled indicators.

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{UI1.png}
    \caption{This is a view of the User Interface, the Analysts
    used for part 1 of the Ground Truth creation. The extracted
    Indicators can be seen marked in a blue rectangle.}
    \label{fig:UI1}
\end{figure*}


\section{LANCE Generalizability}
\label{app:Generalizability}

\begin{table*}
\resizebox{\linewidth}{!}{%
\centering
\begin{tabular}{|l|ccccc|ccccc|ccccc|}
\hline
\textbf{Type} & \multicolumn{5}{c|}{\textbf{Precision}} & \multicolumn{5}{c|}{\textbf{Recall}} & \multicolumn{5}{c|}{\textbf{F1-Score}} \\
 & \textbf{GPT} & \textbf{Llama} & \textbf{Nemotron} & \textbf{Gemini} & \textbf{Gemma} & \textbf{GPT} & \textbf{Llama} & \textbf{Nemotron} & \textbf{Gemini} & \textbf{Gemma} & \textbf{GPT} & \textbf{Llama} & \textbf{Nemotron} & \textbf{Gemini} & \textbf{Gemma} \\
\hline
URL    & 0.97 & 0.71 & 0.80 & 0.97 & 0.90 & 0.99 & 0.35 & 0.52 & 0.98 & 0.84 & 0.98 & 0.47 & 0.63 & 0.97 & 0.87 \\
Domain & 0.96 & 0.83 & 0.76 & 0.94 & 0.75 & 0.94 & 0.78 & 0.78 & 1.00 & 0.77 & 0.95 & 0.80 & 0.77 & 0.97 & 0.76 \\
HASH   & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 0.86 & 1.00 & 0.99 & 0.99 & 1.00 & 0.93 & 1.00 & 0.99 & 0.99 \\
IP     & 1.00 & 1.00 & 1.00 & 1.00 & 0.99 & 0.95 & 0.99 & 0.68 & 0.98 & 0.95 & 0.97 & 0.99 & 0.81 & 0.99 & 0.97 \\
\hline
\textbf{Total} & \textbf{{0.98}} & \textbf{0.92} & \textbf{0.90} & \textbf{{0.98}} & \textbf{0.93} & \textbf{0.98} & \textbf{0.76} & \textbf{0.80} & \textbf{{0.99}} & \textbf{0.91} & \textbf{{0.98}} & \textbf{0.83} & \textbf{0.85} & \textbf{{0.98}} & \textbf{0.92} \\
\hline
\end{tabular}
}
\caption{Comparison of the LANCE implementation using GPT, Llama, Nvidia Nemotron, Gemini, and Gemma on IoC Classification.}
\label{tab:LLM_eval}
\end{table*}

\section{Complimentary Material}

\begin{table}[h!]
\centering
\begin{tabular}{|l|cc|cc|cc|}
\hline
\textbf{Type} & \multicolumn{2}{c|}{\textbf{Precision}} & \multicolumn{2}{c|}{\textbf{Recall}} & \multicolumn{2}{c|}{\textbf{F1-Score}} \\
 & \textbf{GPT} & \textbf{GPT*} & \textbf{GPT} & \textbf{GPT*}& \textbf{GPT} & \textbf{GPT*}\\
\hline
fqdn & 0.88 & 0.97 &  0.95 & 0.96  & 0.91 & 0.96  \\
\textbf{Total} & \textbf{0.97} & \textbf{0.99} & \textbf{0.99} & \textbf{0.99} &  \textbf{0.98} & \textbf{0.99}  \\
\hline
\end{tabular}
\caption{Comparison of GPT performance when assuming that the over 70\% of FP domains that are FP because of an ambiguous definition of what is an IoC, are considered TP}
\label{tab:GPT_with_without_FP}
\end{table}

\begin{table}[h]
    \centering
    \begin{tabular}{lccccc}
        \hline
        \textbf{Indicator Type} & \textbf{P5} & \textbf{P10} & \textbf{P20} & \textbf{P40} & \textbf{P50} \\
        \hline
        URL  & 0.6667  & 0.6923  & 1.0000  & 1.0000  & 1.0000 \\
        FQDN  & 0.3750  & 0.4286  & 0.8571  & 0.9500  & 1.0000 \\
        Hash  & 0.9524  & 1.0000  & 1.0000  & 1.0000  & 1.0000 \\
        IPv4  & 1.0000  & 1.0000  & 1.0000  & 1.0000  & 1.0000 \\
        \hline
    \end{tabular}
    \caption{Performance metrics (P5, P10, P20, P40, P50) for different indicator types based on pairs of Analysts in part 1. Each column represents the maximum average agreement on reports that are in that percentile. }
    \label{tab:agreement_percentiles_part1}
\end{table}

\begin{table*}[h]
    \centering
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{l|ccc|ccc|ccc|ccc}
        \hline
        \multirow{2}{*}{Method} & \multicolumn{3}{c}{IP} & \multicolumn{3}{c}{Hash} & \multicolumn{3}{c}{URL} & \multicolumn{3}{c}{Domain} \\
        \cline{2-13}
        & Precision & Recall & F1 & Precision & Recall & F1 & Precision & Recall & F1 & Precision & Recall & F1 \\
        \hline
        GoodFATR \cite{GoodFATR}& \textcolor{red}{0.9787} & \textbf{\textcolor[rgb]{0,0.6,0}{1.0000}} & 0.9892 & \textcolor{red}{0.9388} & \textbf{\textcolor[rgb]{0,0.6,0}{0.9817}} & 0.9598 & 0.4706 & 0.8000 & 0.5926 & 0.4383 & \textbf{\textcolor[rgb]{0,0.6,0}{1.0000}} & 0.6094 \\
        
        ioc-extractor \cite{ioc_extractor} & \textcolor{red}{0.9787} & \textbf{\textcolor[rgb]{0,0.6,0}{1.0000}} & 0.9892 & \textcolor{red}{0.9388} & \textbf{\textcolor[rgb]{0,0.6,0}{0.9817}} & 0.9598 & 0.5652 & 0.6500 & 0.6047 & \textcolor{red}{0.4011} & \textbf{\textcolor[rgb]{0,0.6,0}{1.0000}} & \textcolor{red}{0.5726} \\
        
        AlienVault & \textbf{\textcolor[rgb]{0,0.6,0}{1.0000}} & 0.9891 & 0.9945 & 0.8522 & 0.9665 & 0.9057 & \textcolor{red}{0.0238} & \textbf{\textcolor[rgb]{0,0.6,0}{0.1000}} & \textcolor{red}{0.0385} & 0.8222 & \textcolor{red}{0.5211} & 0.6379 \\

        \hline

        GF methodology & \textcolor{red}{0.9787} & \textbf{\textcolor[rgb]{0,0.6,0}{1.0000}} & 0.9892 & \textcolor{red}{0.9388} & \textbf{\textcolor[rgb]{0,0.6,0}{0.9817}} & 0.9598 & 0.4545 & \textcolor{red}{0.5000} & 0.4762 & 0.5071 & \textbf{\textcolor[rgb]{0,0.6,0}{1.0000}} & 0.6730 \\
        
        RegEx + VT (th=1) & \textbf{\textcolor[rgb]{0,0.6,0}{1.0000}} & 0.9891 & 0.9945 & 0.9753 & 0.4907 & 0.6537 & 0.7500 & 0.9375 & 0.8333 & 0.7634 & \textbf{\textcolor[rgb]{0,0.6,0}{1.0000}} & 0.8658 \\

        RegEx + VT (th=5) & \textbf{\textcolor[rgb]{0,0.6,0}{1.0000}} & \textcolor{red}{0.2391} & \textcolor{red}{0.3860} & \textbf{\textcolor[rgb]{0,0.6,0}{0.9870}} & \textcolor{red}{0.4720} & \textcolor{red}{0.6366} & 0.8889 & \textcolor{red}{0.5000} & 0.6400 & \textbf{\textcolor[rgb]{0,0.6,0}{0.9710}} & 0.9437 & 0.9572 \\
        
        RegEx + VT (th=0-5) & \textbf{\textcolor[rgb]{0,0.6,0}{1.0000}} & 0.9737 & 0.9867 & \textbf{\textcolor[rgb]{0,0.6,0}{0.9870}} & 0.4810 & 0.6468 & 0.9000 & 0.9000 & \textbf{\textcolor[rgb]{0,0.6,0}{0.9000}} & 0.9706 & 0.9296 & \textbf{\textcolor[rgb]{0,0.6,0}{0.9851}} \\
        
        \hline
        
        GPT & \textbf{\textcolor[rgb]{0,0.6,0}{1.0000}} & \textbf{\textcolor[rgb]{0,0.6,0}{1.0000}} & \textbf{\textcolor[rgb]{0,0.6,0}{1.0000}} & 0.9847 & \textbf{\textcolor[rgb]{0,0.6,0}{0.9817}} & \textbf{\textcolor[rgb]{0,0.6,0}{0.9832}} & \textbf{\textcolor[rgb]{0,0.6,0}{1.0000}} & 0.8000 & 0.8889 & 0.9589 & 0.9859 & 0.9722 \\
        \hline
    \end{tabular}
    }
    \caption{Precision, Recall, and F1-score for different Methods of Ground Truth IoC Extraction}
    \label{tab:GT_creation_method_eval}
\end{table*}


\begin{table}[h]
    \centering
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{|l|cc|cc|cc|}
        \hline
        \multirow{2}{*}{\textbf{Type}} & \multicolumn{2}{c|}{\textbf{Agree}} & \multicolumn{2}{c|}{\textbf{Disagree}} & \multicolumn{2}{c|}{\textbf{Ratio}} \\
        \cline{2-7}
        & \textbf{All} & \textbf{2 Analysts} & \textbf{All} & \textbf{2 Analysts} & \textbf{All}& \textbf{2 Analysts} \\
        \hline
        URL  & 187   & 189  & 32 & 30  & 0.8539 & 0.8630 \\
        FQDN  & 243   & 255  & 46  & 34  & 0.8408   & 0.8824 \\
        Hash  & 308  & 308  & 2   & 2   & 0.9935   & 0.9935 \\
        IPv4  & 92   & 97   & 5  & 0   & 0.9485  & 1.0000 \\
        CVE  & 10   & 10   & 1   & 1   & 0.9091   & 0.9091 \\
        \hline
        \textbf{Total} & 840   & 859  & 86   & 67  & 0.9071  & 0.9276 \\
        \hline
    \end{tabular}
    }
    \caption{Comparison of Agreement Statistics for Different Types based on All 3 Labels, and 2 Analysts in Part 1 of the Junior Analyst Experiment}
    \label{tab:merged_agreement_stats_part1}
\end{table}

\begin{table}[h]
    \resizebox{\linewidth}{!}{%
    \centering
    \begin{tabular}{l|cc|cc|cc}
        \toprule
        \multirow{2}{*}{\textbf{Type}} & \multicolumn{2}{c|}{\textbf{Agree}} & \multicolumn{2}{c|}{\textbf{Disagree}} & \multicolumn{2}{c}{\textbf{Ratio}} \\
        \cline{2-7}
        & \textbf{All} & \textbf{2 Analysts} & \textbf{All} & \textbf{2 Analysts} & \textbf{All} & \textbf{2 Analysts} \\
        \hline
        URL  & 142  & 145  & 6   & 3   & 0.9595  & 0.9797 \\
        FQDN  & 241  & 244  & 7   & 4   & 0.9718  & 0.9839 \\
        Hash  & 394  & 395  & 9   & 8   & 0.9777  & 0.9801 \\
        IPv4  & 60   & 60   & 0   & 0   & 1.0000  & 1.0000 \\
        \hline
        \textbf{Total} & 843 & 850 & 22  & 15  & 0.9746  & 0.9827 \\
        \bottomrule
    \end{tabular}
    }
    \caption{Comparison of Agreement Statistics for Different Types based on All 3 Labels vs. 2 Analysts in Part 2 of the Junior Analyst Experiment}
    \label{tab:agreement_stats_part2}
\end{table}


\begin{table}[h]
    \resizebox{\linewidth}{!}{%
\centering
\begin{tabular}{l|cc|cc|cc}
\toprule
\multirow{2}{*}{\textbf{Type} }& \multicolumn{2}{c|}{\textbf{Precision}} & \multicolumn{2}{c|}{\textbf{Recall}} & \multicolumn{2}{c}{\textbf{F1 Score}} \\
                  & \textbf{GPT} & \textbf{IoC Searcher} & \textbf{GPT} & \textbf{IoC Searcher} & \textbf{GPT} & \textbf{IoC Searcher} \\
\hline
IP      & 0.87 & 0.83 & 1.00 & 1.00 & 0.93 & 0.91 \\
Hash    & 0.90 & 0.90 & 1.00 & 1.00 & 0.95 & 0.95 \\
URL     & 0.73 & 0.65 & 1.00 & 1.00 & 0.84 & 0.79 \\
Domain  & 0.93 & 0.71 & 1.00 & 1.00 & 0.96 & 0.83 \\
\hline
\textbf{Total} & 0.88 & 0.76 & 1.00 & 1.00 & 0.94 & 0.87 \\

\bottomrule
\end{tabular}
}
\caption{Performance Comparison between GPT and IoC Searcher for prompt evaluation}
    \label{tab:prompt_eval}
\end{table}

\begin{table}[h]
    \resizebox{.95\linewidth}{!}{%
    \centering
    \begin{tabular}{l|cc|cc|cc}
        \toprule
        \multirow{2}{*}{\textbf{Type}} & \multicolumn{2}{c|}{\textbf{Precision}} & \multicolumn{2}{c|}{\textbf{Recall}} & \multicolumn{2}{c}{\textbf{F1}} \\
        \cline{2-7}
        & GPT & Analysts & GPT & Analysts & GPT & Analysts \\
        \hline
        url  & \textbf{0.9686} & 0.9632 & \textbf{0.9872} & 0.9231 & \textbf{0.9778} & 0.9427 \\
        fqdn & \textbf{0.9595} & 0.9064 & 0.9432 & \textbf{0.9631} & \textbf{0.9513} & 0.9339 \\
        hash & 0.9968 & \textbf{0.9984} & \textbf{1.0000} & 0.9984 & \textbf{0.9984} & \textbf{0.9984} \\
        ip4  & \textbf{1.0000} & \textbf{1.0000} & 0.9485 & \textbf{1.0000} & 0.9735 & \textbf{1.0000} \\
        \hline
        \textbf{Total} & \textbf{0.9826} & 0.9688 & \textbf{0.9773} & 0.9740 & \textbf{0.9799} & 0.9714 \\
        \bottomrule
    \end{tabular}
    }
    \caption{Performance comparison between GPT and Analysts on Part1}
    \label{tab:GPT_Analyst_performance_on_part1}
\end{table}

\begin{table}[h]
    \resizebox{.95\linewidth}{!}{%
    \centering
    \begin{tabular}{l|cc|cc|cc}
        \toprule
        \multirow{2}{*}{\textbf{Type}} & \multicolumn{2}{c|}{\textbf{Precision}} & \multicolumn{2}{c|}{\textbf{Recall}} & \multicolumn{2}{c}{\textbf{F1}} \\
        \cline{2-7} 
        & GPT & Analysts & GPT & Analysts & GPT & Analysts \\
        \hline
        url  & 0.9709 & \textbf{0.9852} & \textbf{1.0000} & \textbf{1.0000} & 0.9852 & \textbf{0.9926} \\
        fqdn & 0.7710 & \textbf{0.7782} & 0.9619 & \textbf{0.9857} & 0.8559 & \textbf{0.8697} \\
        hash & 0.9950 & \textbf{0.9987} & \textbf{1.0000} & 0.9913 & \textbf{0.9975} & 0.9950 \\
        ip4  & \textbf{1.0000} & \textbf{1.0000} & \textbf{1.0000} & \textbf{1.0000} & \textbf{1.0000} & \textbf{1.0000}  \\
        \hline
        \textbf{Total} & 0.9500 & \textbf{0.9547} & \textbf{0.9940} & 0.9925 & 0.9715 & \textbf{0.9733} \\
        \bottomrule
    \end{tabular}
    }
    \caption{Performance comparison between GPT and Analysts on Part2}
    \label{tab:GPT_Analyst_performance_on_part2}
\end{table}

\begin{table}[h!]
\centering
\begin{tabular}{|l|c|c|c|c|}
\hline
\textbf{Method} & \textbf{Count} & \textbf{VT1}& \textbf{VT5}& \textbf{GPT}  \\
\hline
 \textbf{VT1} & 2574 & 0 & 335 & 496 \\
 \textbf{VT5} & 2574 & 335 & 0 & 496 \\
 \textbf{GPT} & 2492 & 496 & 496 & 0 \\
\hline
\end{tabular}
\caption{Evaluation of AspIoC training and fine-tuning experiments on GT}
\end{table}

\begin{table}[h!]
\centering
\begin{tabular}{|l|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c|}{\textbf{Training Experiment}} & \multicolumn{2}{c|}{\textbf{Finetuning Experiment}}  \\
\cline{2-5}
& Accuracy & F1 & Accuracy & F1 \\
\hline
 \textbf{VT1} & 0.5169 & 0.3408 & 0.5169 & 0.3408 \\
 \textbf{VT5} & 0.5169 & 0.3408 & 0.5169 & 0.3408 \\
 \textbf{GPT} & 0.5169 & 0.3408 & 0.5169 & 0.3408 \\
\hline
\end{tabular}
\caption{Comparison of datasets created with VT1, VT5, and GPT, for the training/finetuning of AspIoC}
\end{table}

\begin{table*}[]
    \resizebox{\linewidth}{!}{%
    \centering
    \begin{tabular}{|l|cc|ccc|ccc|ccc|ccc|ccc|}
        \hline
        \multirow{2}{*}{Method} & Labeled & Unlabeled  & \multicolumn{3}{c}{IP} & \multicolumn{3}{c}{Hash} & \multicolumn{3}{c}{URL} & \multicolumn{3}{c|}{Domain} &\multicolumn{3}{c|}{Total} \\
        \cline{4-18}
        &Indicators&Indicators& Precision & Recall & F1 & Precision & Recall & F1 & Precision & Recall & F1 & Precision & Recall & F1 & Precision & Recall & F1 \\
        \hline
        
        IoC Searcher \cite{GoodFATR} & 1806 & - & 0.987 & \textbf{1.000} & \textbf{0.994} & 0.994 & \textbf{1.000} & 0.997 & 0.699 & \textbf{1.000} & 0.823 & 0.523 & \textbf{1.000} & 0.687 & 0.792 & \textbf{1.000} & 0.884 \\

        IoC extractor \cite{ioc_extractor} & 1752 & 217 & 0.981 & \textbf{1.000} & 0.990 & 0.994 & \textbf{1.000} & 0.997 & 0.706 & 0.496 & 0.583 & 0.551 & 0.993 & 0.706 & 0.817 & 0.907 &  0.859\\

        IoC finder \cite{STIXnet , iocfinder} & 1872 & 52 & 0.981 & \textbf{1.000} & 0.990 & 0.994 & \textbf{1.000} & 0.997 & 0.690 & 0.851 & 0.762 & 0.525 & \textbf{1.000} & 0.689 & 0.793 & 0.974 &  0.874\\
        \hline
    \end{tabular}
    }
    \caption{Performance comparison of eight ground truth creation methods across four IoC types (IP, hash, URL, domain) and overall, using precision, recall, and F1 score. IoC Searcher exhibits near-perfect recall but low precision due to excessive false positives. VirusTotal-based methods vary depending on the chosen threshold, with threshold 1|5 offering more balanced results but lower coverage. The LANCE pipeline achieves the highest F1 score overall (97.6\%), demonstrating strong performance across all indicator types while providing excellent coverage.}
    \label{tab:IoC_extraction_methods_eval}
\end{table*}

\begin{figure*}[ht]
    \centering
    \resizebox{\linewidth}{!}{%
    \includegraphics[width=0.7\textwidth]{plots/fp_fn_row.pdf}
    }
    \caption{False positive and false negative categories identified in IoC extraction by IoC Searcher and AlienVault. IoC Searcher shows higher false positives in benign strings such as file paths, while AlienVault primarily fails by including IoCs not found in the report or omitting indicators entirely.}

    \label{fig:fp_fn_combined}
\end{figure*}

\section{Naive Prompt}



Extract all IoC URLs from the following report. Make sure you extracted ALL IoC URLs, but you did not include any false positives. Give me all IoC URLs in a CSV format:

==> Chapters/XRelatedWork.tex <==


\section{Related work} \label{sec:RelatedWork}

The effectiveness of automated Indicator of Compromise (IoC) extraction tools is intrinsically tied to the quality and reliability of the ground truth (GT) datasets used during their development and evaluation. While numerous state-of-the-art tools have been proposed, employing a wide range of techniques from rule-based systems to deep learning and graph-based approaches, the creation of GT datasets remains a significant bottleneck. Existing methods for GT generation often rely on manual labeling, supplemented by automated techniques such as regular expressions, VirusTotal validation, and curated lists. However, these approaches face limitations in scalability, consistency, and adaptability to the dynamic nature of cybersecurity threats. In this section, we review the landscape of automated IoC extraction tools and analyze the methodologies employed for GT dataset creation, underscoring the pressing need for a scalable and reliable GT dataset, a gap that this paper aims to address. In Table~\ref{tab:ioc_tools} we see 18 prominent IoC extraction tools, the technique they use to extract and label the IoCs, the methods the authors implemented to create the ground truth for those tools, as well as the size of those tools, where that information was available. Finally, in the table are shown the available Artifacts of the tools, as well as whether the tool was reproducible. The artifacts were either found in a public repository from the authors or shared by the authors after we contacted them. We contacted all authors by email two times, with two weeks between each attempt. The difficulty in reproducibility of published work has been studied by Olszewski et al. \cite{Reproducability} and documented by other authors in the IoC extraction field \cite{GoodFATR}.


\begin{comment}

\subsection{Automated IoC Extraction Tools} \label{subsec:AutomatedIoCExtractionTools}

Various approaches have been developed to extract Indicators of Compromise (IoCs) from unstructured threat intelligence sources. These methods can be broadly categorized based on the techniques they employ: rule-based systems, natural language processing (NLP), machine learning (ML), deep learning (DL), and graph-based deep learning.

    

\subsubsection{Rule-Based IoC Extraction}


Rule-based systems rely on predefined patterns and rules for IoC extraction. 
IoC Searcher, by Caballero et al. \cite{GoodFATR}, employs modular pipelines with regular expressions enhanced by validation functions to extract IoCs from unstructured threat reports, ensuring high recall by filtering benign indicators. However, its validation relied on a very limited set of ground truth IoCs, which undermines the robustness and generalizability of the approach. The code and dataset of IoC Searcher were available and easily reproducible.
STIXnet \cite{STIXnet} is another system that extracts Indicators of Compromise (IoCs) such as IPs, hashes, and CVEs using a dedicated rule-based module that leverages regular expressions tailored to IoC structures. By integrating this with NLP-enhanced modules and an evolving Knowledge Base, STIXnet enables comprehensive and automated extraction of all STIX-compliant threat intelligence entities and their relationships from CTI reports. Even though the ground truth dataset for this paper was not available, we were able to reproduce the underlying IoC extraction tool IoC finder, as it was publicly available and did not require any training \cite{iocfinder}.
In addition, ioc-extractor and IoCParser, both open-source tools, leverage rule-based extraction methods to identify IoCs \cite{ioc_extractor, iocparser}. These tools are widely used in public IoC sharing forums due to their accessibility.

\subsubsection{Natural Language Processing (NLP)-Based Approaches}

NLP-based methods leverage linguistic structures and semantic patterns to identify IoCs within textual data. 
ChainSmith applies tailored NLP techniques to extract IoCs from threat intelligence reports and classify them into stages of malicious campaigns, addressing challenges such as obfuscation and diverse technical writing styles \cite{ChainSmith}. 
TIMiner by Zhao et al. \cite{TIMiner} also employs NLP techniques, combining word embeddings with syntactic dependency parsing to extract IoCs, including unseen types, from social media. By integrating domain tags, TIMiner creates domain-specific CTIs, demonstrating high accuracy in both CTI domain classification and IoC extraction.  
Another notable approach by Xiao employs generic named entity recognition (NER) tools in its first phase and a word2vec-based domain-specific classifier in its second phase \cite{Two-phase_System}. While this system identifies cybersecurity concepts and IoCs without relying on extensively annotated datasets, its evaluation was limited to only 435 ground truth IoCs, which raises concerns about the comprehensiveness and scalability of its validation.

\subsubsection{Machine Learning (ML)-Based Approaches}

Machine learning methods involve training models on labeled datasets to automatically identify IoCs. 
IoCMiner utilizes regular expression rules to extract IoCs from social media platforms like Twitter and Pastebin \cite{IoCMiner}. The system integrates a reputation model to evaluate source credibility and employs a random forest classifier to filter relevant content, thereby improving the reliability of extracted IoCs. The code and dataset of IoCMiner were available and reproducible.
Gharibshah implementation employs transfer learning and word embeddings to extract IPs from security forums, minimizing reliance on extensive labeled data \cite{Extracting_actionable_information}. It uses contextual and user-profile features to distinguish malicious entities and classify security-related threads, demonstrating strong generalization capabilities. 
Twiti integrates machine learning classifiers with NLP techniques to process Twitter data, utilizing contextual features like keywords and n-grams to identify IoCs with high precision \cite{Twiti}. Even though the code for Twiti was available, the tool could not be reproduced as the ground truth dataset was not available.
IoC-Stalker employs sentence transformers to analyze textual and contextual features of posts in underground forums. Then it implements a Random Forest Classifier for the classification of the IoCs. It demonstrates the ability to detect malicious IoCs significantly earlier than traditional OSINT methods. The authors of IoC-Stalker shared their code, and even throw the original ground truth dataset was not available, the tool was reproducible. Because the tool was targeted at forum posts and threads, and it used metadata that were not replaceable in the context of threat reports, we could not evaluate this tool on our dataset.

\subsubsection{Deep Learning (DL)-Based Approaches}

Deep learning approaches use advanced neural networks to capture complex patterns in data for IoC extraction. 
Long et al. \cite{Collecting_Indicators} applied a neural network model with a sequence-labeling architecture to extract IoCs from cybersecurity articles. By combining Bi-LSTM with multi-head self-attention mechanisms, it achieves high performance in token-level and contextual IoC identification. 
Another system, iACE, leverages dependency parsing and graph mining techniques to extract semantic relationships between IoCs and context terms, demonstrating scalability and high precision \cite{iACE}. 
AITI employs a hybrid deep learning approach combining convolutional neural networks (CNNs) with BERT embeddings to extract actionable threat intelligence (TI) from unstructured text \cite{AITI}. By leveraging the contextual understanding provided by BERT and the feature extraction capabilities of CNNs, AITI achieves high performance in TI extraction. 
AspIoC adopts a multi-component architecture, combining character-level and contextual feature extraction with DistillBERT for aspect-level text polarity classification, attaining state-of-the-art performance \cite{AspIoC}. Due to the lack of the dataset that AspIoC used for training, this work was not reproducible, even though part of the code was available. 
STIOCS employs an active learning-based semi-supervised framework that combines deep learning with domain-specific heuristics to efficiently label IoCs, significantly reducing the reliance on large annotated datasets \cite{STIOCS}. The system iteratively refines predictions using a human-in-the-loop approach, enabling scalability while maintaining high accuracy. The code for most functions of STIOCS is available, but the original truth dataset with extracted and labeled IoCs is not, making its reproduction unfeasible.
Zhou et al. \cite{Automatic_Identification} introduce a BiLSTM-CRF model with an attention mechanism to extract IoCs from unstructured cybersecurity reports. It leverages token spelling features and pre-trained embeddings to enhance recognition of low-frequency IoCs, achieving high precision and recall with minimal annotated data. 
CTI View employs a hybrid model combining BERT, BiLSTM, GRU, and CRF to extract named entities such as attackers, tools, and campaigns from APT reports \cite{CTI_View}. The system integrates regular expressions and blacklist/whitelist mechanisms for IoC validation and demonstrates strong performance in building structured threat intelligence for APT knowledge graphs.

\subsubsection{Graph-Based Deep Learning Approaches}

Graph-based approaches model relationships among various entities to extract and analyze IoCs. 
HinCTI uses a heterogeneous information network (HIN) with a graph convolutional network (GCN) to identify IoCs, integrating multiple CTI sources to improve accuracy \cite{HinCTI}. 
HINTI employs a similar HIN-based method, incorporating a multi-granular attention mechanism for IoC extraction \cite{HINTI}. By quantifying interdependencies among IoCs, HINTI enables tasks such as IoC ranking, attack modeling, and vulnerability analysis, providing deeper insights into threat intelligence. The authors of HINTI have shared the code implementation of the tool, but due to the lack of proper documentation and the ground truth dataset, we were not able to reproduce it.


This categorization demonstrates the diversity of automated IoC extraction methods, reflecting the significant advancements in rule-based, ML, DL, and graph-based techniques. Despite these developments, IoC extraction remains a challenging and unsolved problem, with each approach facing limitations in generalization, scalability, or accuracy. Continued research is essential to address these gaps and improve the reliability of automated IoC extraction across diverse and evolving threat intelligence sources.

\end{comment}



\begin{table*}[ht!]
\centering
\renewcommand{\arraystretch}{1.2}
    \resizebox{\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Technique}} & \textbf{IoC extraction} & \multicolumn{6}{c|}{\textbf{Ground Truth (GT) Creation Methods}} & \multicolumn{2}{c|}{\textbf{GT Size}} & \multicolumn{2}{c|}{\textbf{Availability}} & \multirow{2}{*}{\textbf{Usability}}\\ \cline{3-12}
&  \textbf{Tool} & \textbf{Manual} & \textbf{VT} & \textbf{RegEx} & \textbf{Forums} & \textbf{Lists} & \textbf{Unsupervised} & \textbf{Malicious} & \textbf{Not Malicious} & \textbf{Code} & \textbf{Dataset} & \\
\hline
\multirow{2}{*}{Rule Based} & IoC Searcher \cite{GoodFATR} & \fulldot & & & & & & 29 & 77 & \checkmark & \checkmark & \checkmark \\
& STIXnet \cite{STIXnet} & \fulldot & & & & & & - & - & \checkmark &   & \checkmark \\
\hline
\multirow{3}{*}{NLP} & ChainSmith \cite{ChainSmith} & \fulldot & & & & & & 6,264 & - &   &   &  \\
& TIMiner \cite{TIMiner} & & & \checkmark & & & \checkmark & - & - &   &   &  \\
& Xiao \cite{Two-phase_System} & ? & & & & & & 435 & -  &   &   &  \\
\hline
\multirow{4}{*}{Machine Learning} 
& IoCMiner \cite{IoCMiner} & \emptydot & \checkmark & & & & & 45 & 297 & \checkmark & \checkmark  & \checkmark \\
& Gharibshah \cite{Extracting_actionable_information} & ? & \checkmark & & & & & 14,268 & -  &   &   &  \\
& Twiti \cite{Twiti} & \emptydot & \checkmark & & & \checkmark & & 50,653 & - & \checkmark &   &   \\
& IoC Stalker \cite{IoCStalker} & & \checkmark & \checkmark & & & & 63,903 & 439,586 & \checkmark &   & \checkmark \\
\hline
\multirow{7}{*}{Deep Learning} 
& Long et al. \cite{Collecting_Indicators} & ? & & & & & & 69,032 & -  &   &   &   \\
& iACE \cite{iACE} & \fulldot & & \checkmark & \checkmark & & & 1,500 & 3,000   &   &   &   \\
& AITI \cite{AITI} & ? & & & & & & 1,782 & 1,782   &   &   &  \\
& AspIOC \cite{AspIoC} & & \checkmark & \checkmark & & & & 50,235 & 50,185  & \checkmark &   &  \\
& STIOCS \cite{STIOCS} & ? & & \checkmark & \checkmark & & & 5,922 & -   & \checkmark &   &   \\
& Zhou et al. \cite{Automatic_Identification}& ? & & & & & & 69,032 & -   &   &   &   \\
& CTI View \cite{CTI_View}& ? & & \checkmark & \checkmark & \checkmark & & 17,364 & -   &   &   &   \\
\hline
\multirow{2}{*}{Graph-based DL} & HinCTI \cite{HinCTI} & \halfdot & \checkmark & & \checkmark & & & 11,340 & -   &   &   &   \\
& HINTI \cite{HINTI} & ? & & & & & & 30,000 & - & \checkmark &   &   \\
\hline
\end{tabular}
}
\caption{Analysis of IoC extraction tools and their corresponding ground truth (GT) generation methods. The tools are grouped by their underlying extraction technique. Each tool is annotated with the methods that were used for ground truth creation. Where available, dataset sizes for malicious and non-malicious samples are included, along with whether the labeled dataset and or the code implementation are accessible. Finally, the reproducibility of each tool is marked in the final column.}
\label{tab:ioc_tools}
\end{table*}



\subsection{Ground Truth Generation Methods}
\label{subsec:GTgenerationMethods}

Ground truth (GT) creation is a critical component in evaluating the performance of IoC extraction methods. To analyze the different GT creation techniques, we included peer-reviewed papers from conferences and journals that represented state-of-the-art approaches based on their effectiveness and accuracy. Papers that did not perform IoC extraction, those that were reviews of the field, or those that focused on extracting IoCs from structured data rather than unstructured text were excluded from the analysis.

The categories for GT creation methods: manual labeling, VirusTotal (VT)-based validation, regular expression (RegEx)-based matching, curated lists, unsupervised methods, and information sourced from open forums, were derived from patterns observed in the literature. Each category is further illustrated with examples of papers that employed the respective methods, highlighting the diverse strategies used to generate ground truth data.

Table~\ref{tab:ioc_tools} presents an overview of IoC extraction tools and their corresponding ground truth creation methods. It categorizes the tools by their underlying techniques, such as rule-based, NLP, machine learning, deep learning, and graph-based deep learning, and highlights the specific GT creation methods they employ, along with the dataset sizes for malicious and non-malicious samples, where they were disclosed.

\subsubsection{Manual Ground Truth Labeling}

Over 80\% of the IoC extraction methods we examined rely heavily on manual efforts to create ground truth datasets and 57\% of those used only manual IoC extraction to generate their ground truth. Manual labeling is not just a common practice but the backbone of ground truth creation in this domain, reflecting the lack of universally effective automated solutions and benchmark datasets. These approaches involve human expertise to label IoCs, ensuring high precision. Rule-based systems such as IoC Searcher and IoCMiner depend on manual annotations to validate their outputs \cite{GoodFATR, IoCMiner}. Similarly, NLP-based tools such as ChainSmith and the system proposed by Xiao manual GT creation to evaluate their efficacy \cite{ChainSmith, Two-phase_System}. In the machine learning domain, Twiti and Gharibshah's approach employs manual labeling alongside other methods. Many deep learning models, including the one proposed by Long et al., by Zhou et al, iACE, AITI, STIOCS, and CTI View, also depend on manually curated datasets 
\cite{Collecting_Indicators,iACE,STIOCS,CTI_View,Automatic_Identification}. In graph-based deep learning approaches, HinCTI and HINTI similarly rely on manually labeled data \cite{HinCTI,HINTI}.
While manual ground truth creation ensures high precision by leveraging human expertise, it is time-consuming, expensive, and prone to scalability challenges as datasets grow larger. Moreover, manual labeling is susceptible to subjective biases, which can impact the consistency and generalizability of the resulting datasets.


\subsubsection{VirusTotal-Based Validation}

VirusTotal (VT) is a widely used tool for validating IoCs against a repository of malware data and is often integrated as part of the IoC extraction pipeline. However, the threshold for considering an IoC malicious varies across different implementations, reflecting the absence of a standardized approach. These thresholds significantly influence the precision and recall of IoC extraction systems. In our search, we found that 35\% of the examined models incorporate VirusTotal in their ground truth extraction process. ML-based methods such as that proposed by Gharibshah, Twiti, and IoC Stalker \cite{IoCStalker} leverage VT to cross-validate their IoC predictions \cite{Twiti,Extracting_actionable_information}. In the deep learning category, AspIOC integrates VT results to refine its GT datasets \cite{AspIoC}. Graph-based method HinCTI also use VT to enhance the accuracy of their extracted IoCs \cite{HinCTI}.
While VT provides a broad and frequently updated repository for IoC validation, it is prone to errors, often producing false positives and false negatives. These inaccuracies, along with the variability in maliciousness thresholds, can undermine the reliability of systems that depend heavily on VT. 

\subsubsection{Regular Expression (RegEx)-Based Matching}

Regular Expression(RegEx) matching is a common technique for identifying IoCs through pattern matching in textual data. While effective, it is typically used in conjunction with other methods, such as manual validation or curated lists, to create a comprehensive ground truth dataset. This combination ensures higher accuracy and reliability, addressing the limitations of RegEx in handling complex or ambiguous patterns on its own. NLP-based tools such as TIMiner employ RegEx to extract IoCs directly from reports \cite{TIMiner}. In machine learning, IoC Stalker \cite{IoCStalker} integrates RegEx for GT creation, while deep learning systems like iACE, AspIOC, STIOCS, and CTI View utilize RegEx to create their GT datasets \cite{iACE,AspIoC,STIOCS,CTI_View}.
However, RegEx often introduces a high number of false positives, such as misclassifying file names or other textual patterns as domains. This lack of contextual understanding necessitates significant post-processing or manual validation, limiting its standalone effectiveness in IoC extraction.

\subsubsection{Open Source Forums}

Open-source forums and underground communities are valuable sources of data used to complement other ground truth-creation methods. These forums are typically utilized in conjunction with manual validation to ensure the accuracy and reliability of IoC datasets. Tools like iACE, STIOCS, and CTI View leverage information from such forums to gather diverse IoC examples, which are then manually reviewed and processed for inclusion in GT datasets \cite{iACE,STIOCS,CTI_View}. Graph-based approaches like HinCTI also rely on these sources to improve the diversity and authenticity of their GT datasets \cite{HinCTI}.
However, data from these sources often contains significant noise and inaccuracies, including false positives or outdated IoCs. Without rigorous validation, such issues can introduce errors into the ground truth datasets, potentially undermining their quality and reliability.



\subsubsection{Curated Lists}

Curated lists of known IoCs or benign Indicators serve as another method for GT creation. Like RegEx, curated lists are rarely used in isolation to create a ground truth dataset. Instead, they are typically combined with other methods, such as manual and RegEx extraction or VT-based checks, to ensure comprehensive and reliable GT datasets. ML-based tools such as Twiti use such lists to validate their predictions \cite{Twiti}. Deep learning approaches, including CTI View, also incorporate curated lists for IoC validation \cite{CTI_View}.
While curated lists provide a reliable starting point, they are inherently static and struggle to keep pace with the dynamic nature of evolving threats. Additionally, their dependency on manual updates can lead to incomplete or outdated entries, limiting their effectiveness in identifying emerging IoCs.

\subsubsection{Unsupervised Methods}

Unsupervised methods for GT creation involve algorithms that automatically cluster or identify IoCs without requiring labeled data. NLP-based tools like TIMiner use unsupervised techniques alongside RegEx to extract IoCs by labeling indicators that appear in close proximity to specific keywords associated with malicious activities \cite{TIMiner}. 
While this targeted approach reduces the dependence on manual labeling and increases scalability, it can lead to inaccuracies, particularly when the surrounding context is ambiguous or misleading. 

\begin{tcolorbox}[boxsep=-0.5mm, boxrule=0.4mm]
\textbf{Takeaway:} Ground truth creation methods vary significantly across IoC extraction tools, but manual labeling overwhelmingly dominates as the most trusted approach. Despite advancements and implementations of techniques such as RegEx, VT validation, curated lists, and unsupervised learning, manual labeling remains indispensable in most cases because it ensures the reliability and precision of GT datasets, which are essential for training, evaluating, and refining IoC extraction tools. This underscores the pressing need for highly reliable GT datasets, as their quality and availability directly influence the advancement of IoC extraction research and its impact on practical cybersecurity solutions.
\end{tcolorbox}

\begin{comment}
    

\subsection{Motivating Examples}
\label{subsec:MotivatingExamples}





\begin{figure*}[ht]
    \centering
    \resizebox{\linewidth}{!}{%
    \includegraphics[width=0.7\textwidth]{plots/fp_fn_row.pdf}
    }
    \caption{False positive and false negative categories identified in IoC extraction by IoC Searcher and AlienVault. IoC Searcher shows higher false positives in benign strings such as file paths, while AlienVault primarily fails by including IoCs not found in the report or omitting indicators entirely.}

    \label{fig:fp_fn_combined}
\end{figure*}


False positives (FPs) in Indicators of Compromise (IoCs) not only hinder the effectiveness of automated extraction tools but also impose significant challenges on cybersecurity workflows. These inaccurate IoCs often stem from misclassifications by existing tools, where benign artifacts such as filenames, placeholder text, or fragmented strings are mistakenly identified as malicious. Such inaccuracies lead to operational inefficiencies, increasing the time and resources spent investigating harmless entities while critical threats go unnoticed. In this subsection, we present concrete examples of FP IoCs produced by a state-of-the-art extractor, highlighting specific cases where these misclassifications occur. These examples serve to underscore the pressing need for more precise and robust IoC extraction methodologies, and they motivate the contributions of this paper in addressing these limitations.

Figure \ref{fig:fp_fn_combined} provides an overview of the false positives (FPs) and false negatives (FN) identified by IoC Searcher \cite{GoodFATR} and AlienVault \cite{AlienVault} when analyzing 10 cybersecurity reports. The targeted reports were published by known companies in the field in 2024 and were obtained from AlienVault's database \cite{AlienVault}, where a dataset of IoCs extracted from the reports is also available. IoC Searcher is one of the most recent automated IoC extraction tools with publicly available code \cite{GoodFATR}. The ground truth for this analysis was meticulously extracted by two PhD students, ensuring high accuracy in identifying the actual Indicators of Compromise (IoCs). A total of 517 IoCs were manually identified, offering a robust baseline for evaluating the performance of IoC Searcher.

The Figure categorizes FPs into distinct categories, revealing a total of 126 misclassifications from IoC Searcher, thus setting the precision of the tool to 80.5\%. Among these, the most frequent FP category, "not malicious," accounts for 52 instances. These cases arise when benign entities such as URLs, domains, and hashes are incorrectly flagged as malicious. This overreporting of benign data significantly inflates the workload for analysts, as they must manually verify and discard these erroneous IoCs, thereby diverting attention from actual threats.

Another prominent category is "file path," which contributed 22 FPs. Misclassifications in this category involve benign file names or paths mistakenly identified as malicious domains and URLs. This highlights a limitation in the tool’s contextual analysis, as it fails to differentiate between file-related strings and domains. Similarly, "tld" (top-level domain) misclassifications, with 14 occurrences, indicate instances where TLDs were incorrectly flagged as compromised domains, further emphasizing the need for improved domain analysis in IoC extraction tools.

Less frequent but still notable are FPs categorized under "incorrect type", with 10 instances. These errors suggest a misinterpretation of the data’s context, leading the tool to extract irrelevant or incorrectly classified information. For instance, references to threat names may inadvertently identify IoC domains, even though they are not domains and they are unrelated to the malicious activity reported.

A common occurrence (8 instances) of FPs was the misclassification of references to companies reporting the attack as IoCs, even though they are unrelated to the malicious activity.

Additional FPs, such as "segment of Indicator" (14 instances), "placeholder" (2 instances), CVEs related to other attacks (2 instances), and "typos in the report" (2 instances), reflect challenges posed by inconsistent formatting and human errors in report generation. These categories underscore the limitations of automated tools in handling subtle nuances such as incomplete indicators, placeholder text, or typographical errors in the source documents.

When examining the IoC dataset provided from AlienVault \cite{AlienVault}, we see that 55 indicators in the dataset do not appear in the corresponding reports. This phenomenon is mainly caused by the fact that AlineVault includes in the dataset indicators that are relevant to the report, but do not appear in it, like different versions of file hashes (SHA1$\,\to\,$SHA256). These, along with some Indicators that are labeled with incorrect types and a few that are not malicious, set the Precision of AlienVault on this dataset to 87.4\%. 

Further research into the Alien Vault dataset, we saw that there were 67 false negative indicators, setting the recall to 87\%, 60 of which were not found in any form in the dataset.

The findings presented in Figure \ref{fig:fp_fn_combined} underscore the critical need for advancements in IoC extraction technologies. The variety and volume of FPs and FNs highlight gaps in current methodologies, particularly in their ability to interpret context and mitigate errors stemming from benign artifacts or formatting inconsistencies. These motivating examples form the basis for the contributions in this paper, which aim to support the development of more robust and precise extraction techniques to reduce false positives and enhance the operational efficiency of cybersecurity workflows.


\end{comment}
